Turbulence modulation in dense liquid-solid channel flow

We investigate the mechanisms by which inertial solid particles modulate turbulence and alter the fluid mass transport in dense turbulent liquid-solid flows. To this end, we perform Euler-Lagrange simulations at friction Reynolds number 180, particle friction Stokes number 7.9, particle-to-fluid density ratio 8.9, and particle volume fraction ranging from 1% up to 12%. We show that the mechanisms underpinning the flow modulation are two fold: (I) the increase of the suspension's apparent kinematic viscosity with increasing solid volume fraction and (II) turbulence modulation through the particle feedback force. For solid volume fraction below 3%, the increase of the suspension's apparent kinematic viscosity by the disperse particles accounts for most of the flow modification, namely, the reduction of turbulent fluctuations, reduction of the bulk fluid velocity, and increase of friction coefficient. In denser channels, the particle feedback force leads to greater reduction of bulk fluid velocity and increase of friction coefficient than can be accounted for solely based on the increased apparent kinematic viscosity. In these cases, particle stress significantly alters the stress balance, to a point where it exceeds the Reynolds stress at solid volume fraction 12%.

==> sections/Simulation_Initialization.tex <==
\section{Simulation Configuration}

\begin{multicols}{2}

To understand the affect of increasing volume fraction in the onset of turbulence modulation a particle laden channel flow at friction Reynolds 180 is studied. The friction Reynolds number is defined as:

\begin{equation}
    Re_{\tau} = u_{\tau}h/\nu
\end{equation}

Increasing volume fraction is expected to have an increasing affect on modulating the turbulence. This is because the mass loading will increase with volume fraction and have a greater affect through momentum exchange. To ensure that this affect is isolated, the scaled particle diameter is held constant at 4, defined as $d_{p}^{+}=d_{p} u_{\tau}/nu$, the Stokes number, defined as $St^{+}=t_{0} u_{\tau}/\nu$, is held constant at 7.871, and the particle to fluid density ratio, $\rho_{p}/\rho{f}$, is held constant at 8.889. The varied volume fraction, and thereby mass loading, is achieved only through a change in the number of particle, which otherwise have the same properties. This information is summarised in table \ref{tab:Phy_Param}.

As this study is interested in the modulation of turbulence by particles it is necessary to first understand a channel flow at $Re_\tau = 180$ both for comparison of statistics and for use when injecting particles into a turbulent channel for observation of modulation.

\end{multicols}

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
         Parameter & Case 1 & Case 2 & Case 3 & Case 4 & Case 5 \\
         $d_{p}^{+}$ & N/A & 4 & 4 & 4 & 4 \\
         $St^{+}$ & N/A & 7.871 & 7.871 & 7.871 & 7.871\\
         $VFP_{avg}$ & N/A & 0.01 & 0.03 & 0.06 & 0.12\\
         $nbrp$ & 0 & 1.17e+5 & 5.31e+5 & 1.07e+6 & 2.12e+6\\
         $M_{l}$ & 0 & 0.0889 & 0.2667 & 0.5333 & 1.067\\
        \end{tabular}
    \caption{Physical Parameters}
    \label{tab:Phy_Param}
\end{table}

\begin{multicols}{2}

All five simulation cases will be simulated using the same domain size. This is $L_{x} = 4 \pi h$, $L_{y} = 2h$, $L_{z} = 4/3 \pi h$, where h is the channel half height. The channel half height is set as 0.045. The discretization is also the same in all cases and is 256 points in the stream-wise direction, 128 points in the wall-normal direction, and 168 points in the cross-stream direction. The grid is spaced uniformly in the stream-wise and cross-stream directions, while the grid is stretched according to a hyperbolic tangent function with a stretching factor of 1.8 such that $\Delta y^{+}_{min} = 0.5$.

Before beginning any particle laden simulations it is first necessary to conduct a single phase simulation at friction Reynolds 180 defined as:
\begin{equation}
    Re_{\tau} = u_{\tau}h/\nu
\end{equation}

Where $u_{\tau}$ is the friction velocity, defined as $\sqrt{\tau_{w}/\rho_{f}}$ and $\nu$ is the fluid kinematic viscosity.

This is done to match the value used by \textcolor{blue}{Kim and Moin}, until it reaches statistically stationary state. The stationary state will be validated using data from \textcolor{blue}{Kim and Moin} to ensure close agreement. Once this simulation has reached stationary state particles will be injected into the flow to begin particle laden simulations. Shown in \textcolor{blue}{figure} is the mean streamwise velocity from the single phase simulation plotted alongside the data from \textcolor{blue}{Kim and Moin}. 

\end{multicols}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Images/Mean_Velocity_Profiles/u_m_Single_Phase.eps}
    \caption{Mean Velocity, lines correspond to simulation data, symbols correspond to data from \textcolor{blue}{Kim and Moin}}
    \label{fig:Single_Phase_um}
\end{figure}

\begin{multicols}{2}

The simulation data closely matches the behavior observed by \textcolor{blue}{Kim and Moin}, as well as matcing the expected viscous layer and log layer relations. Together these results indicate that the simulation has reached stationary state. Shown in \textcolor{blue}{figure} is the velocity fluctuations in the streamwise, cross-stream, and wall-normal directions. 

\end{multicols}

\begin{figure}
    \includegraphics[width=\linewidth]{Images/RMS_Profiles/RMS_Single_Phase.eps}
    \caption{Velocity fluctuations, Lines correspond to simulation data, symbols correspond to data from \textcolor{blue}{Kim and Moin}}
    \label{fig:Single_Phase_RMS}
\end{figure}

\begin{multicols}{2}

The data can be seen to be in good agreement for all three fluctuations, and this supports the conclusion that the flow has reached statistically stationary state, and that particles can be injected into the flow.

Upon completion of the single phase simulation the particle-laden flows are initialized by injecting particles of the chosen diameter and density in an array of size equal to the domain size with inter-particle spacing such that the volume fraction within the array is equal to the chosen average volume fraction.

Table one shows the parameters investigated in this study. Cases one and two use varying particle diameter to investigate the effect of increasing Stokes number. By increasing the particle diameter while maintaining particle density and average volume fraction the mass loading is kept constant. This leads to a drop in total particle number and allows for rapid simulations in case 2. Cases four and five have a constant particle diameter of $d_{p}^{+} = 4$, as in case two, but the particle density is increased. This has the effect of increasing both the Stokes number and the mass loading. In case 5 the volume fraction is also increased to six percent. This significantly increases the mass loading. This is done to further investigate the effect of increasing Stokes number and in case five to separate the mass loading from the Stokes number.

\end{multicols}

\begin{table}[h]
    \centering
    \begin{tabular}{c|c|c|c|c|c}
         Parameter & Case 1 & Case 2 & Case 3 & Case 4 & Case 5 \\
         $N_{x}$ & 256 & 256 & 256 & 256 & 256\\
         $N_{y}$ & 128 & 128 & 128 & 128 & 128\\
         $N_{z}$ & 168 & 168 & 168 & 168 & 168\\
         $\Delta x^{+}$ & 10 & 10 & 10 & 10 & 10\\
         $\Delta y_{min}^{+}$ & 0.5 & 0.5 & 0.5 & 0.5 & 0.5\\
         $\Delta z^{+}$ & 5 & 5 & 5 & 5 & 5 \\
         
    \end{tabular}
    \caption{Simulation Parameters}
    \label{tab:my_label}
\end{table}

